On the Generalization Limitation of On-Policy Distillation for Post-RL Consolidation

Multi-teacher on-policy distillation (MOPD) extends on-policy distillation (OPD) to consolidate capabilities from multiple teachers. Although prior work reports near-perfect in-distribution (IND) distillation performance, we find that this can mask incomplete capability consolidation beyond the supervised distribution. A preliminary study on synthetic reasoning shows that OPD does not fully transfer teachers' generalization capabilities. We then extend this investigation to real-world tasks, evaluating extrapolative and compositional generalization across mathematical reasoning, coding, agent, and long-context capabilities using Qwen3 models. Across extrapolative settings, OPD and MOPD reach 96.04-102.73% of their teachers' IND scores. Yet their out-of-distribution (OOD) scores remain 2.45-16.25% below the base model's. Across three compositional settings, MOPD improves IND performance over the base model, but its performance on composed tasks as OOD remains 18.19-24.34% below that of the best teachers. To understand these gaps, we examine teacher capability and data coverage as two potential bottlenecks. Jointly alleviating these bottlenecks eliminates OOD forgetting in our experiments and suggests the potential for generalization beyond the teacher. (M)OPD also reduces OOD forgetting on average relative to its reinforcement learning (RL) baselines. Analysis of the associated update geometry reveals smaller and more spectrally concentrated updates on average than those of the RL baselines, along with greater shared update structure under MOPD. Motivated by these findings, we propose geometry-based patching and base-preserving replay to improve OOD performance while largely preserving IND performance. Our findings identify a blind spot in capability consolidation via (M)OPD, highlighting the need for algorithms that explicitly support OOD retention and generalization.

==> opd-fonts/width96.tex <==
% Generated horizontal-width variants of the original template fonts.
% Width 96%, height 100%. No negative tracking; nominal word spacing unchanged.
% Computer Modern math fonts and embedded figure fonts are not remapped.
\DeclareFontFamily{T1}{opdcmr}{}
\pdfmapline{+opdecrm0500 SFRM0500 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrm0500.pfb}
\pdfmapline{+opdecrm0600 SFRM0600 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrm0600.pfb}
\pdfmapline{+opdecrm0700 SFRM0700 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrm0700.pfb}
\pdfmapline{+opdecrm0800 SFRM0800 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrm0800.pfb}
\pdfmapline{+opdecrm0900 SFRM0900 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrm0900.pfb}
\pdfmapline{+opdecrm1000 SFRM1000 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrm1000.pfb}
\pdfmapline{+opdecrm1095 SFRM1095 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrm1095.pfb}
\pdfmapline{+opdecrm1200 SFRM1200 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrm1200.pfb}
\pdfmapline{+opdecrm1440 SFRM1440 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrm1440.pfb}
\pdfmapline{+opdecrm1728 SFRM1728 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrm1728.pfb}
\pdfmapline{+opdecrm2074 SFRM2074 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrm2074.pfb}
\pdfmapline{+opdecrm2488 SFRM2488 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrm2488.pfb}
\pdfmapline{+opdecrm2986 SFRM2986 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrm2986.pfb}
\pdfmapline{+opdecrm3583 SFRM3583 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrm3583.pfb}
\DeclareFontShape{T1}{opdcmr}{m}{n}{<-5.5> opd-fonts/opdecrm0500
  <5.5-6.5> opd-fonts/opdecrm0600
  <6.5-7.5> opd-fonts/opdecrm0700
  <7.5-8.5> opd-fonts/opdecrm0800
  <8.5-9.5> opd-fonts/opdecrm0900
  <9.5-10.475> opd-fonts/opdecrm1000
  <10.475-11.475> opd-fonts/opdecrm1095
  <11.475-13.2> opd-fonts/opdecrm1200
  <13.2-15.84> opd-fonts/opdecrm1440
  <15.84-19.009999999999998> opd-fonts/opdecrm1728
  <19.009999999999998-22.81> opd-fonts/opdecrm2074
  <22.81-27.369999999999997> opd-fonts/opdecrm2488
  <27.369999999999997-32.845> opd-fonts/opdecrm2986
  <32.845-> opd-fonts/opdecrm3583}{}
\pdfmapline{+opdecsl0500 SFSL0500 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsl0500.pfb}
\pdfmapline{+opdecsl0600 SFSL0600 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsl0600.pfb}
\pdfmapline{+opdecsl0700 SFSL0700 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsl0700.pfb}
\pdfmapline{+opdecsl0800 SFSL0800 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsl0800.pfb}
\pdfmapline{+opdecsl0900 SFSL0900 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsl0900.pfb}
\pdfmapline{+opdecsl1000 SFSL1000 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsl1000.pfb}
\pdfmapline{+opdecsl1095 SFSL1095 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsl1095.pfb}
\pdfmapline{+opdecsl1200 SFSL1200 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsl1200.pfb}
\pdfmapline{+opdecsl1440 SFSL1440 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsl1440.pfb}
\pdfmapline{+opdecsl1728 SFSL1728 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsl1728.pfb}
\pdfmapline{+opdecsl2074 SFSL2074 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsl2074.pfb}
\pdfmapline{+opdecsl2488 SFSL2488 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsl2488.pfb}
\pdfmapline{+opdecsl2986 SFSL2986 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsl2986.pfb}
\pdfmapline{+opdecsl3583 SFSL3583 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsl3583.pfb}
\DeclareFontShape{T1}{opdcmr}{m}{sl}{<-5.5> opd-fonts/opdecsl0500
  <5.5-6.5> opd-fonts/opdecsl0600
  <6.5-7.5> opd-fonts/opdecsl0700
  <7.5-8.5> opd-fonts/opdecsl0800
  <8.5-9.5> opd-fonts/opdecsl0900
  <9.5-10.475> opd-fonts/opdecsl1000
  <10.475-11.475> opd-fonts/opdecsl1095
  <11.475-13.2> opd-fonts/opdecsl1200
  <13.2-15.84> opd-fonts/opdecsl1440
  <15.84-19.009999999999998> opd-fonts/opdecsl1728
  <19.009999999999998-22.81> opd-fonts/opdecsl2074
  <22.81-27.369999999999997> opd-fonts/opdecsl2488
  <27.369999999999997-32.845> opd-fonts/opdecsl2986
  <32.845-> opd-fonts/opdecsl3583}{}
\pdfmapline{+opdecti0500 SFTI0500 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfti0500.pfb}
\pdfmapline{+opdecti0600 SFTI0600 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfti0600.pfb}
\pdfmapline{+opdecti0700 SFTI0700 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfti0700.pfb}
\pdfmapline{+opdecti0800 SFTI0800 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfti0800.pfb}
\pdfmapline{+opdecti0900 SFTI0900 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfti0900.pfb}
\pdfmapline{+opdecti1000 SFTI1000 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfti1000.pfb}
\pdfmapline{+opdecti1095 SFTI1095 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfti1095.pfb}
\pdfmapline{+opdecti1200 SFTI1200 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfti1200.pfb}
\pdfmapline{+opdecti1440 SFTI1440 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfti1440.pfb}
\pdfmapline{+opdecti1728 SFTI1728 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfti1728.pfb}
\pdfmapline{+opdecti2074 SFTI2074 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfti2074.pfb}
\pdfmapline{+opdecti2488 SFTI2488 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfti2488.pfb}
\pdfmapline{+opdecti2986 SFTI2986 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfti2986.pfb}
\pdfmapline{+opdecti3583 SFTI3583 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfti3583.pfb}
\DeclareFontShape{T1}{opdcmr}{m}{it}{<-5.5> opd-fonts/opdecti0500
  <5.5-6.5> opd-fonts/opdecti0600
  <6.5-7.5> opd-fonts/opdecti0700
  <7.5-8.5> opd-fonts/opdecti0800
  <8.5-9.5> opd-fonts/opdecti0900
  <9.5-10.475> opd-fonts/opdecti1000
  <10.475-11.475> opd-fonts/opdecti1095
  <11.475-13.2> opd-fonts/opdecti1200
  <13.2-15.84> opd-fonts/opdecti1440
  <15.84-19.009999999999998> opd-fonts/opdecti1728
  <19.009999999999998-22.81> opd-fonts/opdecti2074
  <22.81-27.369999999999997> opd-fonts/opdecti2488
  <27.369999999999997-32.845> opd-fonts/opdecti2986
  <32.845-> opd-fonts/opdecti3583}{}
\pdfmapline{+opdeccc0500 SFCC0500 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfcc0500.pfb}
\pdfmapline{+opdeccc0600 SFCC0600 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfcc0600.pfb}
\pdfmapline{+opdeccc0700 SFCC0700 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfcc0700.pfb}
\pdfmapline{+opdeccc0800 SFCC0800 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfcc0800.pfb}
\pdfmapline{+opdeccc0900 SFCC0900 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfcc0900.pfb}
\pdfmapline{+opdeccc1000 SFCC1000 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfcc1000.pfb}
\pdfmapline{+opdeccc1095 SFCC1095 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfcc1095.pfb}
\pdfmapline{+opdeccc1200 SFCC1200 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfcc1200.pfb}
\pdfmapline{+opdeccc1440 SFCC1440 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfcc1440.pfb}
\pdfmapline{+opdeccc1728 SFCC1728 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfcc1728.pfb}
\pdfmapline{+opdeccc2074 SFCC2074 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfcc2074.pfb}
\pdfmapline{+opdeccc2488 SFCC2488 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfcc2488.pfb}
\pdfmapline{+opdeccc2986 SFCC2986 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfcc2986.pfb}
\pdfmapline{+opdeccc3583 SFCC3583 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfcc3583.pfb}
\DeclareFontShape{T1}{opdcmr}{m}{sc}{<-5.5> opd-fonts/opdeccc0500
  <5.5-6.5> opd-fonts/opdeccc0600
  <6.5-7.5> opd-fonts/opdeccc0700
  <7.5-8.5> opd-fonts/opdeccc0800
  <8.5-9.5> opd-fonts/opdeccc0900
  <9.5-10.475> opd-fonts/opdeccc1000
  <10.475-11.475> opd-fonts/opdeccc1095
  <11.475-13.2> opd-fonts/opdeccc1200
  <13.2-15.84> opd-fonts/opdeccc1440
  <15.84-19.009999999999998> opd-fonts/opdeccc1728
  <19.009999999999998-22.81> opd-fonts/opdeccc2074
  <22.81-27.369999999999997> opd-fonts/opdeccc2488
  <27.369999999999997-32.845> opd-fonts/opdeccc2986
  <32.845-> opd-fonts/opdeccc3583}{}
\pdfmapline{+opdecbx0500 SFBX0500 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbx0500.pfb}
\pdfmapline{+opdecbx0600 SFBX0600 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbx0600.pfb}
\pdfmapline{+opdecbx0700 SFBX0700 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbx0700.pfb}
\pdfmapline{+opdecbx0800 SFBX0800 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbx0800.pfb}
\pdfmapline{+opdecbx0900 SFBX0900 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbx0900.pfb}
\pdfmapline{+opdecbx1000 SFBX1000 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbx1000.pfb}
\pdfmapline{+opdecbx1095 SFBX1095 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbx1095.pfb}
\pdfmapline{+opdecbx1200 SFBX1200 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbx1200.pfb}
\pdfmapline{+opdecbx1440 SFBX1440 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbx1440.pfb}
\pdfmapline{+opdecbx1728 SFBX1728 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbx1728.pfb}
\pdfmapline{+opdecbx2074 SFBX2074 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbx2074.pfb}
\pdfmapline{+opdecbx2488 SFBX2488 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbx2488.pfb}
\pdfmapline{+opdecbx2986 SFBX2986 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbx2986.pfb}
\pdfmapline{+opdecbx3583 SFBX3583 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbx3583.pfb}
\DeclareFontShape{T1}{opdcmr}{bx}{n}{<-5.5> opd-fonts/opdecbx0500
  <5.5-6.5> opd-fonts/opdecbx0600
  <6.5-7.5> opd-fonts/opdecbx0700
  <7.5-8.5> opd-fonts/opdecbx0800
  <8.5-9.5> opd-fonts/opdecbx0900
  <9.5-10.475> opd-fonts/opdecbx1000
  <10.475-11.475> opd-fonts/opdecbx1095
  <11.475-13.2> opd-fonts/opdecbx1200
  <13.2-15.84> opd-fonts/opdecbx1440
  <15.84-19.009999999999998> opd-fonts/opdecbx1728
  <19.009999999999998-22.81> opd-fonts/opdecbx2074
  <22.81-27.369999999999997> opd-fonts/opdecbx2488
  <27.369999999999997-32.845> opd-fonts/opdecbx2986
  <32.845-> opd-fonts/opdecbx3583}{}
\pdfmapline{+opdecrb0500 SFRB0500 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrb0500.pfb}
\pdfmapline{+opdecrb0600 SFRB0600 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrb0600.pfb}
\pdfmapline{+opdecrb0700 SFRB0700 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrb0700.pfb}
\pdfmapline{+opdecrb0800 SFRB0800 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrb0800.pfb}
\pdfmapline{+opdecrb0900 SFRB0900 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrb0900.pfb}
\pdfmapline{+opdecrb1000 SFRB1000 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrb1000.pfb}
\pdfmapline{+opdecrb1095 SFRB1095 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrb1095.pfb}
\pdfmapline{+opdecrb1200 SFRB1200 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrb1200.pfb}
\pdfmapline{+opdecrb1440 SFRB1440 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrb1440.pfb}
\pdfmapline{+opdecrb1728 SFRB1728 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrb1728.pfb}
\pdfmapline{+opdecrb2074 SFRB2074 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrb2074.pfb}
\pdfmapline{+opdecrb2488 SFRB2488 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrb2488.pfb}
\pdfmapline{+opdecrb2986 SFRB2986 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrb2986.pfb}
\pdfmapline{+opdecrb3583 SFRB3583 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfrb3583.pfb}
\DeclareFontShape{T1}{opdcmr}{b}{n}{<-5.5> opd-fonts/opdecrb0500
  <5.5-6.5> opd-fonts/opdecrb0600
  <6.5-7.5> opd-fonts/opdecrb0700
  <7.5-8.5> opd-fonts/opdecrb0800
  <8.5-9.5> opd-fonts/opdecrb0900
  <9.5-10.475> opd-fonts/opdecrb1000
  <10.475-11.475> opd-fonts/opdecrb1095
  <11.475-13.2> opd-fonts/opdecrb1200
  <13.2-15.84> opd-fonts/opdecrb1440
  <15.84-19.009999999999998> opd-fonts/opdecrb1728
  <19.009999999999998-22.81> opd-fonts/opdecrb2074
  <22.81-27.369999999999997> opd-fonts/opdecrb2488
  <27.369999999999997-32.845> opd-fonts/opdecrb2986
  <32.845-> opd-fonts/opdecrb3583}{}
\pdfmapline{+opdecbi0500 SFBI0500 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbi0500.pfb}
\pdfmapline{+opdecbi0600 SFBI0600 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbi0600.pfb}
\pdfmapline{+opdecbi0700 SFBI0700 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbi0700.pfb}
\pdfmapline{+opdecbi0800 SFBI0800 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbi0800.pfb}
\pdfmapline{+opdecbi0900 SFBI0900 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbi0900.pfb}
\pdfmapline{+opdecbi1000 SFBI1000 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbi1000.pfb}
\pdfmapline{+opdecbi1095 SFBI1095 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbi1095.pfb}
\pdfmapline{+opdecbi1200 SFBI1200 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbi1200.pfb}
\pdfmapline{+opdecbi1440 SFBI1440 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbi1440.pfb}
\pdfmapline{+opdecbi1728 SFBI1728 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbi1728.pfb}
\pdfmapline{+opdecbi2074 SFBI2074 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbi2074.pfb}
\pdfmapline{+opdecbi2488 SFBI2488 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbi2488.pfb}
\pdfmapline{+opdecbi2986 SFBI2986 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbi2986.pfb}
\pdfmapline{+opdecbi3583 SFBI3583 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbi3583.pfb}
\DeclareFontShape{T1}{opdcmr}{bx}{it}{<-5.5> opd-fonts/opdecbi0500
  <5.5-6.5> opd-fonts/opdecbi0600
  <6.5-7.5> opd-fonts/opdecbi0700
  <7.5-8.5> opd-fonts/opdecbi0800
  <8.5-9.5> opd-fonts/opdecbi0900
  <9.5-10.475> opd-fonts/opdecbi1000
  <10.475-11.475> opd-fonts/opdecbi1095
  <11.475-13.2> opd-fonts/opdecbi1200
  <13.2-15.84> opd-fonts/opdecbi1440
  <15.84-19.009999999999998> opd-fonts/opdecbi1728
  <19.009999999999998-22.81> opd-fonts/opdecbi2074
  <22.81-27.369999999999997> opd-fonts/opdecbi2488
  <27.369999999999997-32.845> opd-fonts/opdecbi2986
  <32.845-> opd-fonts/opdecbi3583}{}
\pdfmapline{+opdecbl0500 SFBL0500 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbl0500.pfb}
\pdfmapline{+opdecbl0600 SFBL0600 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbl0600.pfb}
\pdfmapline{+opdecbl0700 SFBL0700 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbl0700.pfb}
\pdfmapline{+opdecbl0800 SFBL0800 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbl0800.pfb}
\pdfmapline{+opdecbl0900 SFBL0900 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbl0900.pfb}
\pdfmapline{+opdecbl1000 SFBL1000 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbl1000.pfb}
\pdfmapline{+opdecbl1095 SFBL1095 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbl1095.pfb}
\pdfmapline{+opdecbl1200 SFBL1200 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbl1200.pfb}
\pdfmapline{+opdecbl1440 SFBL1440 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbl1440.pfb}
\pdfmapline{+opdecbl1728 SFBL1728 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbl1728.pfb}
\pdfmapline{+opdecbl2074 SFBL2074 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbl2074.pfb}
\pdfmapline{+opdecbl2488 SFBL2488 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbl2488.pfb}
\pdfmapline{+opdecbl2986 SFBL2986 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbl2986.pfb}
\pdfmapline{+opdecbl3583 SFBL3583 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfbl3583.pfb}
\DeclareFontShape{T1}{opdcmr}{bx}{sl}{<-5.5> opd-fonts/opdecbl0500
  <5.5-6.5> opd-fonts/opdecbl0600
  <6.5-7.5> opd-fonts/opdecbl0700
  <7.5-8.5> opd-fonts/opdecbl0800
  <8.5-9.5> opd-fonts/opdecbl0900
  <9.5-10.475> opd-fonts/opdecbl1000
  <10.475-11.475> opd-fonts/opdecbl1095
  <11.475-13.2> opd-fonts/opdecbl1200
  <13.2-15.84> opd-fonts/opdecbl1440
  <15.84-19.009999999999998> opd-fonts/opdecbl1728
  <19.009999999999998-22.81> opd-fonts/opdecbl2074
  <22.81-27.369999999999997> opd-fonts/opdecbl2488
  <27.369999999999997-32.845> opd-fonts/opdecbl2986
  <32.845-> opd-fonts/opdecbl3583}{}
\pdfmapline{+opdecxc0500 SFXC0500 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfxc0500.pfb}
\pdfmapline{+opdecxc0600 SFXC0600 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfxc0600.pfb}
\pdfmapline{+opdecxc0700 SFXC0700 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfxc0700.pfb}
\pdfmapline{+opdecxc0800 SFXC0800 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfxc0800.pfb}
\pdfmapline{+opdecxc0900 SFXC0900 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfxc0900.pfb}
\pdfmapline{+opdecxc1000 SFXC1000 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfxc1000.pfb}
\pdfmapline{+opdecxc1095 SFXC1095 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfxc1095.pfb}
\pdfmapline{+opdecxc1200 SFXC1200 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfxc1200.pfb}
\pdfmapline{+opdecxc1440 SFXC1440 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfxc1440.pfb}
\pdfmapline{+opdecxc1728 SFXC1728 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfxc1728.pfb}
\pdfmapline{+opdecxc2074 SFXC2074 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfxc2074.pfb}
\pdfmapline{+opdecxc2488 SFXC2488 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfxc2488.pfb}
\pdfmapline{+opdecxc2986 SFXC2986 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfxc2986.pfb}
\pdfmapline{+opdecxc3583 SFXC3583 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfxc3583.pfb}
\DeclareFontShape{T1}{opdcmr}{bx}{sc}{<-5.5> opd-fonts/opdecxc0500
  <5.5-6.5> opd-fonts/opdecxc0600
  <6.5-7.5> opd-fonts/opdecxc0700
  <7.5-8.5> opd-fonts/opdecxc0800
  <8.5-9.5> opd-fonts/opdecxc0900
  <9.5-10.475> opd-fonts/opdecxc1000
  <10.475-11.475> opd-fonts/opdecxc1095
  <11.475-13.2> opd-fonts/opdecxc1200
  <13.2-15.84> opd-fonts/opdecxc1440
  <15.84-19.009999999999998> opd-fonts/opdecxc1728
  <19.009999999999998-22.81> opd-fonts/opdecxc2074
  <22.81-27.369999999999997> opd-fonts/opdecxc2488
  <27.369999999999997-32.845> opd-fonts/opdecxc2986
  <32.845-> opd-fonts/opdecxc3583}{}
\pdfmapline{+opdecui0500 SFUI0500 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfui0500.pfb}
\pdfmapline{+opdecui0600 SFUI0600 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfui0600.pfb}
\pdfmapline{+opdecui0700 SFUI0700 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfui0700.pfb}
\pdfmapline{+opdecui0800 SFUI0800 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfui0800.pfb}
\pdfmapline{+opdecui0900 SFUI0900 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfui0900.pfb}
\pdfmapline{+opdecui1000 SFUI1000 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfui1000.pfb}
\pdfmapline{+opdecui1095 SFUI1095 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfui1095.pfb}
\pdfmapline{+opdecui1200 SFUI1200 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfui1200.pfb}
\pdfmapline{+opdecui1440 SFUI1440 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfui1440.pfb}
\pdfmapline{+opdecui1728 SFUI1728 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfui1728.pfb}
\pdfmapline{+opdecui2074 SFUI2074 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfui2074.pfb}
\pdfmapline{+opdecui2488 SFUI2488 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfui2488.pfb}
\pdfmapline{+opdecui2986 SFUI2986 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfui2986.pfb}
\pdfmapline{+opdecui3583 SFUI3583 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfui3583.pfb}
\DeclareFontShape{T1}{opdcmr}{m}{ui}{<-5.5> opd-fonts/opdecui0500
  <5.5-6.5> opd-fonts/opdecui0600
  <6.5-7.5> opd-fonts/opdecui0700
  <7.5-8.5> opd-fonts/opdecui0800
  <8.5-9.5> opd-fonts/opdecui0900
  <9.5-10.475> opd-fonts/opdecui1000
  <10.475-11.475> opd-fonts/opdecui1095
  <11.475-13.2> opd-fonts/opdecui1200
  <13.2-15.84> opd-fonts/opdecui1440
  <15.84-19.009999999999998> opd-fonts/opdecui1728
  <19.009999999999998-22.81> opd-fonts/opdecui2074
  <22.81-27.369999999999997> opd-fonts/opdecui2488
  <27.369999999999997-32.845> opd-fonts/opdecui2986
  <32.845-> opd-fonts/opdecui3583}{}
\pdfmapline{+opdecsc0500 SFSC0500 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsc0500.pfb}
\pdfmapline{+opdecsc0600 SFSC0600 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsc0600.pfb}
\pdfmapline{+opdecsc0700 SFSC0700 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsc0700.pfb}
\pdfmapline{+opdecsc0800 SFSC0800 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsc0800.pfb}
\pdfmapline{+opdecsc0900 SFSC0900 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsc0900.pfb}
\pdfmapline{+opdecsc1000 SFSC1000 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsc1000.pfb}
\pdfmapline{+opdecsc1095 SFSC1095 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsc1095.pfb}
\pdfmapline{+opdecsc1200 SFSC1200 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsc1200.pfb}
\pdfmapline{+opdecsc1440 SFSC1440 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsc1440.pfb}
\pdfmapline{+opdecsc1728 SFSC1728 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsc1728.pfb}
\pdfmapline{+opdecsc2074 SFSC2074 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsc2074.pfb}
\pdfmapline{+opdecsc2488 SFSC2488 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsc2488.pfb}
\pdfmapline{+opdecsc2986 SFSC2986 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsc2986.pfb}
\pdfmapline{+opdecsc3583 SFSC3583 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfsc3583.pfb}
\DeclareFontShape{T1}{opdcmr}{m}{scsl}{<-5.5> opd-fonts/opdecsc0500
  <5.5-6.5> opd-fonts/opdecsc0600
  <6.5-7.5> opd-fonts/opdecsc0700
  <7.5-8.5> opd-fonts/opdecsc0800
  <8.5-9.5> opd-fonts/opdecsc0900
  <9.5-10.475> opd-fonts/opdecsc1000
  <10.475-11.475> opd-fonts/opdecsc1095
  <11.475-13.2> opd-fonts/opdecsc1200
  <13.2-15.84> opd-fonts/opdecsc1440
  <15.84-19.009999999999998> opd-fonts/opdecsc1728
  <19.009999999999998-22.81> opd-fonts/opdecsc2074
  <22.81-27.369999999999997> opd-fonts/opdecsc2488
  <27.369999999999997-32.845> opd-fonts/opdecsc2986
  <32.845-> opd-fonts/opdecsc3583}{}
\pdfmapline{+opdecoc0500 SFOC0500 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfoc0500.pfb}
\pdfmapline{+opdecoc0600 SFOC0600 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfoc0600.pfb}
\pdfmapline{+opdecoc0700 SFOC0700 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfoc0700.pfb}
\pdfmapline{+opdecoc0800 SFOC0800 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfoc0800.pfb}
\pdfmapline{+opdecoc0900 SFOC0900 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfoc0900.pfb}
\pdfmapline{+opdecoc1000 SFOC1000 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfoc1000.pfb}
\pdfmapline{+opdecoc1095 SFOC1095 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfoc1095.pfb}
\pdfmapline{+opdecoc1200 SFOC1200 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfoc1200.pfb}
\pdfmapline{+opdecoc1440 SFOC1440 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfoc1440.pfb}
\pdfmapline{+opdecoc1728 SFOC1728 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfoc1728.pfb}
\pdfmapline{+opdecoc2074 SFOC2074 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfoc2074.pfb}
\pdfmapline{+opdecoc2488 SFOC2488 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfoc2488.pfb}
\pdfmapline{+opdecoc2986 SFOC2986 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfoc2986.pfb}
\pdfmapline{+opdecoc3583 SFOC3583 "0.96 ExtendFont T1Encoding ReEncodeFont" <cm-super-t1.enc <sfoc3583.pfb}
\DeclareFontShape{T1}{opdcmr}{bx}{scsl}{<-5.5> opd-fonts/opdecoc0500
  <5.5-6.5> opd-fonts/opdecoc0600
  <6.5-7.5> opd-fonts/opdecoc0700
  <7.5-8.5> opd-fonts/opdecoc0800
  <8.5-9.5> opd-fonts/opdecoc0900
  <9.5-10.475> opd-fonts/opdecoc1000
  <10.475-11.475> opd-fonts/opdecoc1095
  <11.475-13.2> opd-fonts/opdecoc1200
  <13.2-15.84> opd-fonts/opdecoc1440
  <15.84-19.009999999999998> opd-fonts/opdecoc1728
  <19.009999999999998-22.81> opd-fonts/opdecoc2074
  <22.81-27.369999999999997> opd-fonts/opdecoc2488
  <27.369999999999997-32.845> opd-fonts/opdecoc2986
  <32.845-> opd-fonts/opdecoc3583}{}
\DeclareFontShape{T1}{opdcmr}{b}{scsl}{<->ssub*opdcmr/bx/scsl}{}
\DeclareMicrotypeAlias{opdcmr}{cmr}
\renewcommand{\rmdefault}{opdcmr}
\pdfmapline{+opdbytesans ByteSans-Bold-Width96 <T1-WGL4.enc <opd-fonts/ByteSans-Bold-Width96.ttf}
\DeclareFontFamily{T1}{opdbytesans}{}
\DeclareFontShape{T1}{opdbytesans}{m}{n}{<-> opd-fonts/opdbytesans}{}
\DeclareFontShape{T1}{opdbytesans}{b}{n}{<-> opd-fonts/opdbytesans}{}
\DeclareFontShape{T1}{opdbytesans}{bx}{n}{<-> opd-fonts/opdbytesans}{}
\pdfmapline{+opdbytesansmedium ByteSans-Medium-Width96 <T1-WGL4.enc <opd-fonts/ByteSans-Medium-Width96.ttf}
\DeclareFontShape{T1}{bytesansmedium}{m}{n}{<-> opd-fonts/opdbytesansmedium}{}
\DeclareFontShape{T1}{bytesansmedium}{b}{n}{<-> opd-fonts/opdbytesansmedium}{}
\DeclareFontShape{T1}{bytesansmedium}{bx}{n}{<-> opd-fonts/opdbytesansmedium}{}
\renewcommand{\sfdefault}{opdbytesans}
\normalfont
\endinput

